Adaptive Proof Refinement with LLM-Guided Strategy Selection

Formal verification via theorem proving enables the expressive specification and rigorous proof of software correctness, but it is difficult to scale due to the significant manual effort and expertise required. While Large Language Models (LLMs) show potential in proof generation, they frequently produce incorrect proofs on the first attempt and require additional strategies for iterative refinement. However, existing approaches employ fixed refinement strategies and cannot dynamically choose an effective strategy based on the particular issues in a generated proof, which limits their performance. To overcome this limitation, we introduce Adapt, a novel proof refinement framework that leverages an LLM-guided decision-maker to dynamically select a suitable refinement strategy according to the state of the proof assistant and available context of an incorrect proof. We evaluate Adapt on two benchmarks against four existing methods and find that it significantly outperforms the best baseline on both by proving 16.63% and 18.58% more theorems, respectively. Furthermore, we demonstrate Adapt's generalizability by evaluating it across five different LLMs. We also conduct ablation studies to measure the contribution of each component and compare the trade-offs of alternative decision-maker designs.

==> Makefile <==
JOBNAME      = adapt
LATEXMK      = latexmk
LATEXMKFLAGS = -pdf -jobname=$(JOBNAME) -interaction=nonstopmode -halt-on-error
# keep the next line ONLY if you use minted/gnuplot/etc.
LATEXMKFLAGS += -shell-escape

.PHONY: all haste clean cleanall

all:
	$(LATEXMK) $(LATEXMKFLAGS) main.tex

haste:
	pdflatex $(filter -shell-escape,$(LATEXMKFLAGS)) -jobname=$(JOBNAME) \
	         -interaction=nonstopmode main

clean:
	$(LATEXMK) -c -jobname=$(JOBNAME)

cleanall:
	$(LATEXMK) -C -jobname=$(JOBNAME)


==> examples/case_1.tex <==
\begin{figure}[h]{\textwidth}
\lstset{style=coq}
\begin{lstlisting}
Lemma rotate_right_Ordered_imp v l r :
  Ordered (rotate_right v l r) → Ordered (Node v l r).
Proof.
  destruct l as [|lv ll lr]; eauto 2.
  rewrite !Ordered_iff_Ordered'.
  ...
\end{lstlisting}
\caption{\label{case:1}}
\label{fig:enter-label}
\end{figure}

% 87bcd47f57705bbd967a9825f587cf0043188f23 AVL.v

==> examples/case_2.tex <==
\begin{figure}[h]{\textwidth}
\lstset{style=coq}
\begin{lstlisting}
Lemma envt_dec: forall n n1 H G, env_type n H G -> n1 <= n -> env_type n1 H G.
Proof.
  ...
  eapply valt_dec; eauto. 
Qed.
\end{lstlisting}
\caption{\label{case:2}}
\label{fig:enter-label}
\end{figure}

==> examples/case_3.tex <==
\begin{figure}[h]{\textwidth}
\lstset{style=coq}
\begin{lstlisting}
Lemma L_as_K : forall n, L n = K n << 0.
Proof.
  destruct n as [| n].
  - apply const_unfold.
  - simpl. induction n; simpl; try rewrite IHn; reflexivity.
Qed.
\end{lstlisting}
\caption{\label{case:3}}
\label{fig:enter-label}
\end{figure}
